Information-Theoretic Fairness with A Bounded Statistical Parity Constraint

In this paper, we study an information-theoretic problem of designing a fair representation that attains bounded statistical (demographic) parity. More specifically, an agent uses some useful data $X$ to solve a task $T$. Since both $X$ and $T$ are correlated with some sensitive attribute or secret $S$, the agent designs a representation $Y$ that satisfies a bounded statistical parity and/or privacy leakage constraint, that is, such that $I(Y;S) \leq \epsilon$. Here, we relax the perfect demographic (statistical) parity and consider a bounded-parity constraint. In this work, we design the representation $Y$ that maximizes the mutual information $I(Y;T)$ about the task while satisfying a bounded compression (or encoding rate) constraint, that is, ensuring that $I(Y;X) \leq r$. Simultaneously, $Y$ satisfies the bounded statistical parity constraint $I(Y;S) \leq \epsilon$. To design $Y$, we use extended versions of the Functional Representation Lemma and the Strong Functional Representation Lemma which are based on randomization techniques and study the tightness of the obtained bounds in special cases. The main idea to derive the lower bounds is to use randomization over useful data $X$ or sensitive data $S$. Considering perfect demographic parity, i.e., $\epsilon=0$, we improve the existing results (lower bounds) by using a tighter version of the Strong Functional Representation Lemma and propose new upper bounds. We then propose upper and lower bounds for the main problem and show that allowing non-zero leakage can improve the attained utility. Finally, we study the bounds and compare them in a numerical example. The problem studied in this paper can also be interpreted as one of code design with bounded leakage and bounded rate privacy considering the sensitive attribute as a secret.

==> contents/conclusion_prev.tex <==
We have studied two information-theoretic fairness problems where in both problems we design private and fair representations of the useful data $X$. To design the representations we have used randomization technique which has been used in extending two constructive and important lemmas, the Functional Representation Lemma and the Strong Functional Representation Lemma. We have shown that the randomization technique with these two lemmas leads to simple designs. Considering both problems, we have shown that when the rate $r$ is more than a threshold the obtained designs can be optimal. Specifically, for the first problem when the private data is deterministic function of the task the lower bound is tight.

==> contents/intro_prev.tex <==
%The amount of data generated by interconnected sensors that record and process signals from the physical world, software system, humans and robots is growing rapidly. Direct disclosure of the raw data can cause privacy threats through unauthorized inferences. Thus, privacy mechanisms are required for data disclosure.

In this paper, we consider the scenario illustrated in Fig. \ref{fig:enter-label}, in which random variable (RV) $X$ denotes the useful data and is used to address a task (goal), make a decision, or draw inferences about it. Here, the task is denoted by RV $T$ and we assume that both the useful data and the task are arbitrarily correlated with a private latent attribute denoted by RV $S$. The task, private data, and the useful data are sampled from a joint distribution $P_{S,X,T}$. Since the task $T$ and the useful data $X$ are dependent on the private data $S$, it is not desirable that our inferences be influenced by $S$. Hence, we encode the useful data $X$ to $Y$ and use $Y$ to draw conclusion about the task $T$. We refer to $Y$ as disclosed data and the goal of designing $Y$ is to maximize the mutual information between $Y$ and $T$ (in other words, $Y$ should keep as much as information as possible about the task $T$) while satisfying two constraints. Firstly, $Y$ should be independent of $S$ which corresponds to the perfect privacy constraint. Secondly, it should satisfy the bounded encoding rate constraint where the mutual information between the disclosed data $Y$ and the useful data $X$ should be bounded by a constant, i.e., $I(Y;X)\leq r$. Here, the constant $r$ controls the encoding rate of the useful data $X$. The obtained problem corresponds to a trade-off between the utility, privacy leakage and encoding rate. This trade-off can correspond the \textit{demographic parity gap} problem \cite{zemel}. Furthermore, it can correspond to the privacy-utility trade-off with a bounded rate constraint studied in \cite{gun}.   

Next, we consider a scenario which is inspired by the \textit{conditional fairness bottleneck} problem studied in \cite{vari}. As illustrated in Fig. \ref{ITW1}, the goal is to design $Y$ which maximizes the information about the task $T$ which is not shared by the private data $S$ and $Y$ is independent of $S$. Moreover, the information about the useful data $X$ which is not shared by the private data $S$ and the task $T$ is controlled by a constant. In other words, we want to design $Y$ that maximizes the gray area in Fig. \ref{ITW1} while the areas of $Y$ and $S$ do not intersect which corresponds to the perfect privacy and the black area should be less than a fixed constant which corresponds to the bounded encoding rate.  

\begin{figure}
    \centering
    \begin{tikzpicture}
        \draw[draw=black, fill=gray!5, rounded corners] (-2.8, -1.8) rectangle ++(6.2,4);
        \node at (2.9, -1.5) {agent};
     
        \node[draw, circle] (secret) at (0,1.2) {$S$};
        \node[draw, circle] (data) at (0,0) {$X$};
        \node[draw, circle] (task) at (0, -1.2) {$T$};
        \node[draw, rectangle, rounded corners] (joint) at (-2,0) {$P_{S,X,T}$};
        \node[draw, rectangle, rounded corners] (mechanism) at (2.5,0) {$P_{Y|S,X,T}$};
        \node[draw, circle] (representation) at (4.4,0) {$Y$};
        
        \node at (0, 1.8) {\begin{tabular}{c} \small{sensitive attribute} \\ \small{or secret} \end{tabular}};
        \node at (0.0, 0.55) {\small{data}};
        \node at (0, -0.7) {\small{task}};
        \node at (2.5, 0.65) {\begin{tabular}{c} \small{fairness} \\ \small{mechanism} \end{tabular}};
        \node at (4.4, 0.65) {\begin{tabular}{c} \small{disclosed} \\ \small{representation} \end{tabular}};

        \draw[-stealth] (joint.east) -- (secret.west);
        \draw[-stealth] (joint.east) -- (data.west);
        \draw[-stealth] (joint.east) -- (task.west);

        \draw[-stealth] (data.east) -- (mechanism.west);
        \draw[dashed] (secret.east) -- (mechanism.west);
        \draw[dashed] (task.east) -- (mechanism.west);

        \draw[-stealth] (mechanism.east) -- (representation.west);
    \end{tikzpicture}
    \caption{Data representation with perfect demographic parity problem. We want to design a representation $Y$ of the data $X$ that is useful for the task $T$, is compressed, and contains no information about the sensitive attribute or secret $S$.}
    \label{fig:enter-label}
\end{figure}

% \begin{figure}[]
% 	\centering
% 	\includegraphics[scale = .15]{ISITsys.jpg}
% 	\caption{Demographic parity gap problem. We design $Y$ that maximizes the information about $T$ while satisfying perfect privacy and bounded encoding rate constraints.}
% 	\label{ISITsys}
% \end{figure}
\begin{figure}[]
	\centering
	\includegraphics[scale = .15]{Figs/cfb-vd-perfect.pdf}
	\caption{Information diagram~\cite{yeung1991new} of the CFB with perfect demographic parity. In light gray, we show the relevant information about the task $T$, not shared by the sensitive attribute $S$, that we want the representation $Y$ to maximize. In dark gray, we show the irrelevant information about the data $X$ that we want to constrain. Contrary to the standard CFB~\cite{vari}, we enforce that the representation contains no information about the sensitive attribute (perfect demographic parity or perfect privacy).}
	\label{ITW1}
\end{figure}
The privacy and fairness mechanism design problems have received increased attention in recent years
\cite{gun, vari,zhao2022, zhao2019,zemel, gronowski2023classification,hardt, king3, borz, khodam, Khodam22,kostala,makhdoumi, yamamoto1988rate, sankar, Calmon2}.


Considering fairness mechanism design, in \cite{vari}, a variational approach for learning fair representation is proposed. In more detail, the problem of \textit{conditional fairness bottleneck} is introduced where the trade-off between utility and fairness in terms of mutual information is investigated. The obtained optimization problem is studied using a variational approach based on the Lagrangian. The approach of learning \textit{fair representations} is used in \cite{zhao2019,zemel}, where the goal is to design the representations that minimize the amount of private contents while are informative about the task. 
Two widely used and important definitions for fairness, \textit{demographic parity} and \textit{equalized odds} are introduced in \cite{zemel, hardt, zhao2019}
Moreover, a theoretical trade-off between fairness and utility has been studied in \cite{zhao2022}. Furthermore, another fair representation learning method called the \textit{R{\'e}nyi Fair Information Bottleneck Method} is introduced in \cite{gronowski2023classification}. This method considers constraints for fairness, utility and compression of representation, simultaneously.        

Considering privacy mechanism design, in \cite{borz}, the problem of privacy-utility trade-off considering mutual information both as measures of utility and privacy is studied. It is shown that under the perfect privacy assumption, the optimal privacy mechanism problem can be obtained as the solution of a linear program. In \cite{khodam}, the work \cite{borz} is generalized by relaxing the perfect privacy assumption allowing some small bounded leakage. This result is generalized to a non-invertible leakage matrix in \cite{Khodam22}.

The concept of a privacy funnel is introduced in \cite{makhdoumi}, where the privacy utility trade-off considering log-loss for privacy metric and distortion metric has been studied. In \cite{Calmon2}, fundamental limits of the privacy utility trade-off measuring the leakage using estimation-theoretic guarantees are studied.
In \cite{yamamoto}, a source coding problem with secrecy is studied. Privacy-utility trade-offs considering equivocation as measure of privacy and expected distortion as a measure of utility are studied in both \cite{yamamoto} and \cite{sankar}.
In \cite{kostala}, the \emph{secrecy by design} concept has been introduced and is applied to privacy mechanism and lossless compression design problems. For the privacy problem, bounds on privacy-utility trade-off are derived by using the Functional Representation Lemma. These results are derived under the perfect privacy assumption. The privacy problems considered in \cite{kostala} are generalized in \cite{king3} by relaxing the perfect privacy constraint. Moreover, the problems of fixed length and variable length compression with a certain privacy constraint have been studied in \cite{kostala} and upper and lower bounds on the average length of encoded message have been derived. %These results are derived under the perfect privacy constraint. 
A similar approach has been used in \cite{kostala2}, where in a lossless compression problem the relations between shared key, secrecy, and compression considering perfect secrecy, secrecy by design, maximal leakage, mutual information leakage and local differential privacy have been studied.

   
%correlated with the private data denoted by RV $X$. Furthermore, disclosed data is described by RV $U$. Two scenarios are considered in this work, where in both scenarios, an agent wants to disclose the useful information to a user as shown in Fig.~\ref{ISITsys}. In the first scenario, the agent observes $Y$ and has no direct access to $X$, i.e., the private data is hidden. The goal is to design $U$ based on $Y$ that reveals as much information as possible about $Y$ and satisfies a privacy criterion. We use mutual information to measure utility and privacy leakage. In this work, some bounded privacy leakage is allowed, i.e., $I(X;U)\leq \epsilon$. In the second scenario, the agent has access to both $X$ and $Y$ and can design $U$ based on $(X,Y)$ to release as much information as possible about $Y$ while satisfying the bounded leakage constraint.
 %In particular, we allow bounded privacy leakage, i.e., $I(X;U)\leq\epsilon$.
 %\\
%The privacy mechanism design problem is receiving increased attention in information theory recently. Related works can be found in 
%\cite{Calmon2,yamamoto, sankar,borz, gun,khodam,Khodam22,kostala,issa, makhdoumi, dwork1, calmon4, asoo, Total, issa2}. 
\iffalse
Specifically,  %The concept of maximal leakage has been introduced in \cite{issa} and some bounds on the privacy utility trade-off have been derived. 

%In both \cite{yamamoto} and \cite{sankar}, the privacy-utility trade-off is considered using expected distortion as a measure of utility and equivocation as measure of privacy. 
In \cite{Calmon2}, fundamental limits of the privacy utility trade-off measuring the leakage using estimation-theoretic guarantees are studied.
In \cite{yamamoto}, a source coding problem with secrecy is studied.

Privacy-utility trade-offs considering equivocation as measure of privacy and expected distortion as a measure of utility are studied in both \cite{yamamoto} and \cite{sankar}.
In \cite{borz}, the problem of privacy-utility trade-off considering mutual information both as measures of privacy and utility given the Markov chain $X-Y-U$ is studied. It is shown that under perfect privacy assumption, i.e., $\epsilon=0$, the privacy mechanism design problem can be reduced to a linear program. This work has been extended in \cite{gun} considering the privacy utility trade-off with a rate constraint for the disclosed data.
Moreover, in \cite{borz}, it has been shown that information can be only revealed if $P_{X|Y}$ is not invertible. In \cite{khodam}, we designed privacy mechanisms with a per letter privacy criterion considering an invertible $P_{X|Y}$ where a small leakage is allowed. We generalized this result to a non-invertible leakage matrix in \cite{Khodam22}.
%In \cite{borz}, the problem of maximizing utility, i.e., $I(U;Y)$, under the leakage constraint $I(U;X)\leq \epsilon$ and Markov chain $X-Y-U$ is studied and it is shown that under perfect privacy assumption, i.e., $\epsilon=0$, the privacy mechanism design problem can be reduced to standard linear programming.
\fi
In this paper, in contrast to previous works that rely on variational approaches, we propose a simple and constructive theoretical approach to design a private and fair representation of the useful data, i.e., to design the disclosed data.    
Here, the first problem addresses a fairness design where the demographic parity definition of the fairness is used and the second problem is closely related to the conditional fairness bottleneck \cite{vari}. 
To design the disclosed data in both scenarios we use extended versions of the Functional Representation Lemma and  Strong Functional Representation Lemma derived in \cite{king3}. In \cite{king3}, it is shown that both lemmas  
are constructive and simple helping us to obtain privacy mechanism designs that can be optimal in special cases. In this paper, we use similar techniques used as in \cite{king3} and \cite{kostala} to obtain simple and important private and fair representations. We compare the obtained designs considering different scenarios and show that in special cases they are optimal. 

%Our problem here is closely related to \cite{kostala}, where the problem of \emph{secrecy by design} is studied. Similarly, the two scenarios are considered while the results are however derived under the perfect secrecy assumption, i.e., no leakages are allowed which corresponds to $\epsilon=0$. Bounds on secure decomposition have been derived using the Functional Representation Lemma and new bounds on privacy-utility trade-off for the two scenarios are derived. The bounds are tight when the private data is a deterministic function of the useful data. 

%In the present work, we generalize the privacy problems considered in \cite{kostala} by relaxing the perfect privacy constraint and allowing some leakages. To this end, we extend the Functional Representation Lemma relaxing the independence condition. Additionally, we derive bounds by also extending the Strong Functional Representation Lemma, introduced in \cite{}. Furthermore, in the special case of perfect privacy we find a new upper bound for perfect privacy function by using the \emph{excess functional information} introduced in \cite{}. In the extended version \cite{Amir111}, we compare our new lower and upper bounds with the bounds found in \cite{kostala} when the leakage is zero. %As stated earlier, in \cite{borz}, the problem in first scenario is solved under the perfect privacy assumption.

==> contents/main_results_prev.tex <==
In this section, we derive upper and lower bounds on $g^{r}(P_{S,X,T})$ and $g^{r}_c(P_{S,X,T})$ defined in \eqref{eq:problem_1} and \eqref{eq:problem_2}. For this, we employ similar techniques as used in \cite{king3}.
 More specifically, we use extended versions of the Functional Representation Lemma and the strong Functional Representation Lemma proposed in \cite[Lemma 4]{king3} and \cite[Lemma 5]{king3}, respectively. We emphasize that both lemmas have constructive proof so that it helps us to provide private and fair representation $Y$.
  %which has been used in \cite{kostala}. We first encode the private data $X$ using a one-time pad \cite[Lemma~1]{kostala2}, then encode the RV found by the achievable scheme in \cite[Theorem~1]{maddah1} by using the Functional Representation Lemma and blocks of $CF$ bits. To do so, let us, first recall FRL.
 
 
 
 
% In this section, we first recall the Functional Representation Lemma (FRL) \cite[Lemma~1]{kostala} and Strong Functional Representation Lemma (SFRL) \cite[Theorem~1]{} for discrete $X$ and $Y$. Then we extend them for correlated $X$ and $U$, i.e., $0\leq I(U;X)=\epsilon$ and we call them Extended Functional Representation Lemma (EFRL) and Extended Strong Functional Representation Lemma (ESFRL), respectively.
% \begin{lemma}\label{lemma1} (Functional Representation Lemma \cite[Lemma~1]{kostala}):
% 	For any pair of RVs $(X,Y)$ distributed according to $P_{XY}$ supported on alphabets $\mathcal{X}$ and $\mathcal{Y}$ where $|\mathcal{X}|$ is finite and $|\mathcal{Y}|$ is finite or countably infinite, there exists a RV $U$ supported on $\mathcal{U}$ such that $X$ and $U$ are independent, i.e., we have
% 	\begin{align}\label{c1}
% 	I(U;X)=0,
% 	\end{align}
% 	$Y$ is a deterministic function of $(U,X)$, i.e., we have
% 	\begin{align}
% 	H(Y|U,X)=0,\label{c2}
% 	\end{align}
% 	and 
% 	\begin{align}
% 	|\mathcal{U}|\leq |\mathcal{X}|(|\mathcal{Y}|-1)+1.\label{c3}
% 	\end{align}
% \end{lemma}
%%\begin{proof}
%%	The proof can be found in \cite[Lemma~1]{kostala}.
%%\end{proof}
%\begin{lemma}\label{lemma2} (Strong Functional Representation Lemma \cite[Theorem~1]{}):
%	For any pair of RVs $(X,Y)$ distributed according to $P_{XY}$ supported on alphabets $\mathcal{X}$ and $\mathcal{Y}$ where $|\mathcal{X}|$ is finite and $|\mathcal{Y}|$ is finite or countably infinite with $I(X,Y)< \infty$, there exists a RV $U$ supported on $\mathcal{U}$ such that $X$ and $U$ are independent, i.e., we have
%	\begin{align*}
%	I(U;X)=0,
%	\end{align*}
%	$Y$ is a deterministic function of $(U,X)$, i.e., we have 
%	\begin{align*}
%	H(Y|U,X)=0,
%	\end{align*}
%	$I(X;U|Y)$ can be upper bounded as follows
%	\begin{align*}
%I(X;U|Y)\leq \log(I(X;Y)+1)+4,
%	\end{align*}
%	and 
%	$
%	|\mathcal{U}|\leq |\mathcal{X}|(|\mathcal{Y}|-1)+2.
%	$
%\end{lemma}
%%\begin{proof}
%%	The proof is based on exponential functional representation and can be found in \cite[Th.~1]{}.
%%\end{proof}
%\begin{remark}
%	By checking the proof in \cite[Th.~1]{}, the term $e^{-1}\log(e)+2+\log(I(X;Y)+e^{-1}\log(e)+2)$ can be used instead of $\log(I(X;Y)+1)+4$. 
%\end{remark}
%\begin{lemma}\label{lemma3} (Extended Functional Representation Lemma):
%	For any $0\leq\epsilon< I(X;Y)$ and pair of RVs $(X,Y)$ distributed according to $P_{XY}$, %supported on alphabets $\mathcal{X}$ and $\mathcal{Y}$ where $|\mathcal{X}|$ is finite and $|\mathcal{Y}|$ is finite or countably infinite,
%	 there exists a RV $U$ supported on $\mathcal{U}$ such that the leakage between $X$ and $U$ is equal to $\epsilon$, i.e., we have
%	\begin{align*}
%	I(U;X)= \epsilon,
%	\end{align*}
%	$Y$ is a deterministic function of $(U,X)$, i.e., we have  
%	\begin{align*}
%	H(Y|U,X)=0,
%	\end{align*}
%	and 
%	$
%	|\mathcal{U}|\leq \left[|\mathcal{X}|(|\mathcal{Y}|-1)+1\right]\left[|\mathcal{X}|+1\right].
%	$
%\end{lemma}
%\begin{proof}
%	The proof is provided in Appendix A.
%\end{proof}
%\begin{lemma}\label{lemma4} (Extended Strong Functional Representation Lemma):
%	For any $0\leq\epsilon< I(X;Y)$ and pair of RVs $(X,Y)$ distributed according to $P_{XY}$ %supported on alphabets $\mathcal{X}$ and $\mathcal{Y}$ where $|\mathcal{X}|$ is finite and $|\mathcal{Y}|$ is finite or countably infinite 
%	with $I(X,Y)< \infty$, there exists a RV $U$ supported on $\mathcal{U}$ such that the leakage between $X$ and $U$ is equal to $\epsilon$, i.e., we have
%	\begin{align*}
%	I(U;X)= \epsilon,
%	\end{align*}
%	$Y$ is a deterministic function of $(U,X)$, i.e., we have 
%	\begin{align*}
%	H(Y|U,X)=0,
%	\end{align*}
%	$I(X;U|Y)$ can be  upper bounded as follows 
%	\begin{align*}
%	I(X;U|Y)\leq \alpha H(X|Y)\!+\!(1-\alpha)\!\left[ \log(I(X;Y)+1)\!+\!4\right],
%	\end{align*}
%	and 
%	$
%	|\mathcal{U}|\leq \left[|\mathcal{X}|(|\mathcal{Y}|-1)+2\right]\left[|\mathcal{X}|+1\right],
%	$
%	where $\alpha =\frac{\epsilon}{H(X)}$.
%\end{lemma}
%\begin{proof}
%	The proof is provided in Appendix A.
%\end{proof}
%We provide a lemma in Appendix B, where %we first find a lower bound on $H(U)$ where $U$ satisfies \eqref{c1} and \eqref{c2}, then 
%we show that there exists a RV $U$ that satisfies \eqref{c1}, \eqref{c2} and has bounded entropy. The lemma is a generalization of %\cite[Lemma~2]{kostala} and
%\cite[Lemma~2]{kostala} for dependent $X$ and $U$. 

Before stating the next theorem we derive an important expression for $I(Y;T)$. We have
\begin{align}
I(Y;T)&=I(X,S,T;Y)-I(X,S;Y|T),\nonumber\\&=I(X,S;Y)+I(T;Y|X,S)-I(X,S;Y|T),\nonumber\\&=I(X,S;Y)+H(T|X,S)-H(T|Y,X,S)\nonumber\\ &\ \ -I(X,S;Y|T).\label{key}
\end{align}
Similarly as \cite{kostala} and \cite{king3}, \eqref{key} is an important observation to find lower and upper bounds for $g^{r}(P_{S,X,T})$ and $g^{r}_c(P_{S,X,T})$. %In the next theorem we generalize \cite[Th. 5]{kostala} for dependent $X$ and $U$.
%\begin{theorem}
%	For any $0\leq \epsilon< I(X;Y)$ and pair of RVs $(X,Y)$ distributed according to $P_{XY}$ supported on alphabets $\mathcal{X}$ and $\mathcal{Y}$, if $h_{\epsilon}(P_{XY})>\epsilon$ then we have
%	\begin{align*}
%	H(Y|X)>0.
%	\end{align*}
%	Furthermore, if $H(Y|X)-H(X|Y)=H(Y)-H(X)>0$, then
%	\begin{align*}
%	h_{\epsilon}(P_{XY})>\epsilon.
%	\end{align*}
%\end{theorem}
%\begin{proof}
%	For proving the first part let $h_{\epsilon}(P_{XY})>\epsilon$. Using \eqref{key} we have
%	\begin{align*}
%	\epsilon&< h_{\epsilon}(P_{XY})\leq H(Y|X)+\sup_{U:I(X;U)\leq\epsilon} I(X;U)\\&=H(Y|X)+\epsilon
%	\Rightarrow 0<H(Y|X).
%	\end{align*}
%	For the second part assume that $H(Y|X)-H(X|Y)>0$. Let $U$ be produced by EFRL. Thus, using the construction of $U$ as in Lemma~\ref{lemma3} we have $I(X,U)=\epsilon$ and $H(Y|X,U)=0$. Then by using \eqref{key} we obtain
%	\begin{align*}
%	h_{\epsilon}(P_{XY})&\geq \epsilon\!+\!H(Y|X)\!-\!H(X|Y)+H(X|Y,U)\\&\geq \epsilon\!+\!H(Y|X)\!-\!H(X|Y)>\epsilon.
%	\end{align*}
%\end{proof}
In the next theorem we provide a lower and upper bounds on $g^{r}(P_{S,X,T})$.
\begin{theorem}\label{th.1}
	For any $0\leq r\leq H(X|S)$ and RVs $(X,T,S)$ distributed according to $P_{S,X,T}$ we have
	\begin{align}\label{th2}
	\max\{L_1^{r},L_2,L_3^{r}\}\leq g^{r}(P_{S,X,T})\leq H(T|S),
	\end{align}
	where
	\begin{align*}
	L_1^{r} &= H(T|X,S)+r-H(X,S|T),\\
	L_2 &= H(T|X,S)-\left( \log(I(X,S;T)+1)+4 \right),\\
	L_3^{r} &= H(T|X,S)+r-\alpha H(X,S|T)\\&\!\!\!\!\!\!\!\!-\!\log((1\!-\!\alpha)I(X,S;T)\!+\!\alpha\min\{H(T),H(X,S)\}\!+\!1)\!-\!4,
\end{align*}
and $\alpha=\frac{r}{H(X|S)}$. Moreover, for $H(X|S)\leq r< H(X)$ we have
 \begin{align}\label{th22}
 \max\{{L'}_1^{r},L_2\}\leq g^{r}(P_{S,X,T})\leq H(T|S),
 \end{align}
 where 
 \begin{align*}
 {L'}_1^{r} = H(T|S)-H(S|T)=H(T)-H(S).
 %L_3^{r} &= H(T|X,S)+r-\alpha H(X,S|T)\\&\!\!\!\!\!\!\!\!-\!\log((1\!-\!\alpha)I(X,S;T)\!+\!\alpha\min\{H(T),H(X,S)\}\!+\!1)\!-\!4,
 \end{align*}
%The lower bound in \eqref{th2} is tight if $H(X|Y)=0$, i.e., $X$ is a deterministic function of $Y$. Furthermore, if the lower bound $L_1$ is tight then we have $H(X|Y)=0$. 
\end{theorem}
\begin{sproof}
	The complete proof is provided in Appendix A. By removing the rate constraint we obtain the upper bound. To derive $L_2$ we use the Strong Functional Representation Lemma (SFRL) \cite[Theorem~1]{} with $X\leftarrow (X,S)$, $Y\leftarrow T$, and the output $Z\leftarrow Y$. Using \eqref{key} we have
	\begin{align*}
	I(T;Y)&=H(T|X,S)-I(X,S;Y|T)\\&\geq H(T|X,S)\!-\!\left( \log(I(X,S;T)+1)+4 \right)\!=\!L_2,
	\end{align*} 
	The key idea to achieve $L_1^{r}$ and $L_3^{r}$ is to randomize over the output of the Functional Representation Lemma (FRL) \cite[Lemma1]{kostala} $U$ to produce $U'$. To obtain $L_1^{r}$ let $U$ be the output of the FRL. First, we show that $I(U;X)\leq H(X|S)$. We then construct $U'$ using the randomization technique that is used in \cite[Lemma 4]{king3}. Let $U'=\begin{cases}
	U,\ \text{w.p}.\ \alpha\\
	c,\ \ \text{w.p.}\ 1-\alpha
	\end{cases}$ where $\alpha=\frac{r}{H(X|S)}$. Furthermore, let $Y'$ be produced by the FRL with $S\leftarrow (S,X,U')$ and $X\leftarrow T$. Finally, let $Y=(U',Y')$. We first show that for such $Y$ the constraints $I(S;Y)=0$ and $I(X;Y)\leq r$ are satisfied. Then by using \eqref{key} we obtain $L_1^{r}$. Considering \eqref{key}, the key steps to achieve $L_1^{r}$ are as follows
	\begin{align}
	&I(Y',U';X,S)\!=\!I(U';X,S)\!=\!I(U';S)\!+\!I(U';X|S)\!=\!r,\\
	&H(T|X,S,U',Y')=0.
	\end{align} 
	To derive $L_3^{r}$ we use same $U'$, but to produce $Y'$ we use the conditional SFRL with $S\leftarrow (S,X)|U'$ and $X\leftarrow T$. Next, we find an upper bound on $I(X,S;Y',U'|T)$ in \eqref{key}. Using the upper bound and the fact that $I(X,S;Y',U')=r$ we obtain the lower bound $L_3^{r}$. Finally, to derive ${L'}_1^{r}$ we use the following inequality
	\begin{align*}
	g^{r}(P_{S,X,T})\geq g^{r=H(X|S)}(P_{S,X,T}).
	\end{align*}
\end{sproof}
%\begin{proof}
%aa
%	\end{proof}
\begin{corollary}
	Considering the regime $H(X|S)\leq r < H(X)$, when the private data is a deterministic function of the task $S=f(T)$, the lower bound ${L'}_1^{r}$ is tight.
\end{corollary}
\begin{remark}
	\normalfont
	In \eqref{eq:problem_1}, as we mentioned earlier we have used demographic parity definition of the fairness, however, we can also use equalized odds definition where similar techniques as in Theorem 1 can be used. Due to the limited space we leave this as a future work. 
\end{remark}
\begin{remark}
	\normalfont
	The lower bounds in Theorem 1 can be used to address the rate limited privacy-utility trade-off in \cite{gun} with $r<H(X)$.
\end{remark}
\begin{remark}
	\normalfont
	To derive lower bounds considering the regime $H(X|S)\leq r < H(X)$ we have used the inequality $g^{r}(P_{S,X,T})\geq g^{r=H(X|S)}(P_{S,X,T})$. 
	This bound can be also achieved by using $Y=(U,Y')$ where $U$ is the output of the FRL, since in this regime $U$ satisfies $I(U;X)\leq H(X|S)\leq r$ and $I(U;X,S)=H(X|S)$.
	Moreover, by letting $r=H(X|S)$ we have $L_1^{r}\geq L_3^{r}$. Hence, $L_3^{r}$ is not considered in \eqref{th22}. 
	%Although the lower bound ${L'}_1^{r}$ seems to be a good bound, we can strengthen it, and we leave this as a future work.
\end{remark}
	The key idea to achieve $L_1^{r}$ and $L_3^{r}$ is to randomize over the output of the FRL $U$ to produce $U'$. To see the reason for producing $U'$ we focus on the term $I(Y;X,S)$ in\eqref{key}. 
	The challenge is that using the constraints $I(Y;S)=0$ and $I(Y;X)\leq r$ we have 
	\begin{align*}
	I(Y;X,S)=I(Y;S)+I(Y,X|S)\leq H(X|S)
	\end{align*}
	and somehow we want to make this term as large as possible while satisfying the rate constraint. By producing $U$ we have 
	\begin{align*}
	I(U;X,S)=I(U;S)+I(U,X|S)=H(X|S)
		\end{align*}
	since $I(U;S)=0$ and $H(X|U,S)=0$. But, considering the regime $r\leq H(X|S)$, $U$ does not necessarily satisfies $I(U;X)\leq r$. Hence, we randomize over $U$ so that $I(U';X)$ becomes less than or equal to $r$, however, the utility decreases from $H(X|S)$ to $r$, i.e., $I(U;X,S)=H(X|S)$ and $I(U';X,S)=r$.  
	Thus, The main reason to produce $U'$ is to achieve non-zero utility for the term $I(U';X,S)$ in \eqref{key} while satisfying $I(U';X)\leq r$. Furthermore, we produce $Y'$ to ensure that the term $H(T|X,S,Y)$ in \eqref{key} is zero. Note that $Y'$ does not change the term $I(Y;X,S)$ since it is independent of $(U',X,S)$.
	
	\subsection{Comparison and Discussion}
	In this part, we compare the obtained bounds in Theorem 1.
	To compare $L_1^{r}$ and $L_2$, consider the case where $r$ is small and $H(X,T|S)>>4$, then we have $L_2\geq L_1^{r}$. On other hand, when $H(X,T|S)\leq 4$, we have $L_2\leq L_1^{r}$. To compare $L_2$ and $L_3^{r}$ let $H(X|S)\leq H(X,S|T)$, then we have $L_2\geq L_3^{r}$ since we have
	\begin{align*}
	&r-\alpha H(X,S|T)\leq 0,\\
	&I(X,S;T)\leq (1\!-\!\alpha)I(X,S;T)\!+\!\alpha\min\{H(T),H(X,S)\}.
	\end{align*}      
	A simple example for having $H(X|S)\leq H(X,S|T)$ is to let $T$ be a deterministic function of $S$. On the other hand let $H(X|S)> H(X,S|T)$, ignoring the $\log(\cdot)$ terms (since they have smaller values compared to the other terms) we can have $L_2\leq L_3^{r}$. A simple example is to consider $S=f(T)$. Next, we compare $L_1^{r}$ and $L_3^{r}$. To do so let $0<r<<H(X|S)$ ($r$ is small) and $H(X,S|T)>>4$ then we can have $L_1^{r}\leq L_3^{r}$. In other words, comparing $L_3^{r}$ and $L_1^{r}$, we have decreased the term $H(X,S|T)$ in $L_1^{r}$ by multiplying it by $0\leq\alpha\leq1$, but we get a penalty that corresponds to $\log((1\!-\!\alpha)I(X,S;T)\!+\!\alpha\min\{H(T),H(X,S)\}\!+\!1)\!-\!4$. Intuitively, when $r$ is small $L_3^{r}$ is larger than $L_1^{r}$, but when $r$ grows $L_1^{r}$ becomes larger. Considering the extreme case $r=H(X|S)$ we see that $L_1^{r}\geq L_3^{r}$. Considering $r\geq H(X|S)$, it seems that ${L'}_1^{r}$ is a good candidate since its distance with the upper bound is $H(S|T)$. Furthermore, to achieve it, considering \eqref{key} the term $I(Y;X,S)$ achieves $H(X|S)$ which is its maximum with the constraints $I(Y;S)=0$ and $I(X;Y)\leq r$. 
	\begin{remark}
		\normalfont
		The advantage of $L_1^{r}$ and $L_3^{r}$ compared to $L_2$ is to achieve non-zero utility for the term $I(Y;X,S)$, i.e., the added term corresponding to $r$ in both bounds. For instance, consider a case where $T$ is a function of $X$. In this case, $L_2\leq 0$, however, both bounds $L_1^{r}$ and $L_3^{r}$ can achieve non-zero utility.   
	\end{remark}
	\begin{example}
		Let $r=H(X|S)$ and $H(S|T)<4$. In this case $L_1^{r}$ is dominant and we have $L_1^{r}\geq \max\{L_2^{r},L_3^{r}\}$. The latter follows since we have
		\begin{align*}
		&L_1^{r=H(X|S)}-L_2^{r=H(X|S)}=H(T|S)-H(T|X,S)\\&+\left( \log(I(X,S;T)+1)+4 \right)-H(S|T)\geq 0.
		\end{align*} 
		Furthermore,
		\begin{align*}
		&L_1^{r=H(X|S)}-L_3^{r=H(X|S)}=\\&\log(\min\{H(T),H(X,S)\}+1)+4\geq 0.
		\end{align*} 
	\end{example}
	\subsection{Bounds on $g^{r}_c(P_{S,X,T})$}
	In this part, we derive upper and lower bounds on $g^{r}_c(P_{S,X,T})$ defined in \eqref{eq:problem_2}.
	\begin{theorem}
			For any RVs $(X,T,S)$ distributed according to $P_{S,X,T}$, when $r\geq H(X|T,S)$ we have
			\begin{align}
			g^{r}_c(P_{S,X,T})=H(T|S).
			\end{align}
			Furthermore, when $\log(I(X;T|S)+1)+4\leq r\leq H(X|T,S)$, we have
			\begin{align}\label{chap}
			L_1\leq g^{r}_c(P_{S,X,T})\leq H(T|S)
			\end{align}
			where
			\begin{align}
			L_1 = H(T|S,X)-\log(I(X;T|S)+1)-4.
			\end{align}
	\end{theorem}   
\begin{proof}
	The upper bound can be easily derived since we have
	\begin{align*}
	I(Y;T|S)\leq H(T|S).
	\end{align*}
	When $r\geq H(X|T,S)$, the bounded irrelevant data constraint is satisfied since $I(X;Y|S,T)\leq H(X|S,T)$. Furthermore, let $Y$ be found by the FRL \cite[Lemma 1]{kostala} using $S\leftarrow S$ and $X\leftarrow T$. In this case, we have
	\begin{align}
	I(Y;S)&=0,\\
	H(T|Y,S)&=0.\label{mama}
	\end{align}  
	Furthermore, we have
	\begin{align*}
	I(T;Y|S)=H(T|S),
	\end{align*}
	where in the last line we use \eqref{mama}. Hence, considering $r\geq H(X|T,S)$ we have $g^{r}_c(P_{S,X,T})=H(T|S)$. Next, let $\log(I(X;T|S)+1)+4\leq r\leq H(X|T,S)$. We build $Y$ using the conditional SFRL \cite{}. Thus, $Y$ satisfies 
	\begin{align}
	I(Y;S,X)&=0,\label{3ek}\\
	H(T|S,X,Y)&=0,\label{3ek1}\\
	I(Y;X|T,S)&\leq \log(I(X;T|S)+1)+4.\label{3ek2}
	\end{align}
	Next, we expand $I(Y;X,T|S)$ in two ways. We have
	\begin{align}
	I(Y;X,T|S)=I(Y;T|S)+I(Y;X|S,T)\\\leq I(Y;T|S)+\log(I(X;T|S)+1)+4,\label{esha2}
	\end{align}
	where in the last line we have used \eqref{3ek2}.
	On the other hand,
	\begin{align}
	I(Y;X,T|S)&=I(Y;X|S)+I(Y;T|X,S)\nonumber\\&=H(T|X,S),\label{esha}
	\end{align}
	where in the last line we have used \eqref{3ek} and \eqref{3ek1}. By using \eqref{esha} and \eqref{esha2} we have
	\begin{align}
	I(T;Y|S)\geq H(T|X,S)-\log(I(X;T|S)+1)-4.
	\end{align}
\end{proof}
\begin{corollary}
	When the useful data $X$ is deterministic function of the private data $S$, i.e., $X=f(S)$, the lower bound $L_1$ in \eqref{chap} is tight within $4$ bits.
\end{corollary}
\begin{remark}
	The results in Theorem 2 are obtained considering all the rates $r$ larger than a threshold. The problem with $r$ less than the threshold is left to the extended version of the paper. 
\end{remark}

==> contents/system_prev.tex <==
Let $P_{SXT}$ denote the joint distribution of discrete random variables $S$, $X$ and $T$ defined on finite alphabets $\cal{S}$, $\cal{X}$ and $\cal T$. %We assume that cardinality $|\mathcal{X}|$ is finite and $|\mathcal{Y}|$ is finite or countably infinite.
 We represent $P_{SXT}$ by a matrix defined on $\mathbb{R}^{|\mathcal{S}|\times|\mathcal{X}|\times|\mathcal{T}|}$ and %We assume that $X$ and $Y$are defined on spaces that have the same cardinality, i.e., $|\cal{X}|=|\cal{Y}|=\mathcal{K}$. 
marginal distributions of $S$, $X$ and $T$ by vectors $P_S$, $P_X$ and $P_T$ defined on $\mathbb{R}^{|\mathcal{S}|}$, $\mathbb{R}^{|\mathcal{X}|}$ and $\mathbb{R}^{|\mathcal{T}|}$.
Moreover, discrete RV $Y$ defined on alphabet $\mathcal{Y}$ denotes the fair and private representation of useful data $X$. We refer to $Y$ as disclosed data. 
 %given by the row and column sums of $P_{XY}$. 
%We assume that each element in vectors $P_X$ and $P_Y$ is non-zero. Furthermore, 
%We represent the leakage matrix $P_{X|Y}$ by a matrix defined on $\mathbb{R}^{|\mathcal{X}|\times|\cal{Y}|}$.
%In this work, RVs $X$ and $Y$ denote the private data and the useful data and $U$ describes the disclosed data. 
Here, $X$, $S$, and $T$ denote the useful data, the private attribute, and the task, respectively.
As we mentioned earlier, for the first problem we use demographic parity definition of the fairness. The goal is to design $Y$ that maximizes the information about $T$ while satisfying the perfect privacy and the bounded encoding rate constraint. The first design problem can be stated as follows
\begin{align}
    g^{r}(P_{SXT})&=\sup_{\begin{array}{c} 
	\substack{P_{Y|SXT}:I(Y;S)=0,\\ \ \ \ \ \ \ \ \  I(X;Y)\leq r }
	\end{array}}I(Y;T),
    \label{eq:problem_1}
\end{align} 
The relation between $Y$ and $(S,X,T)$ is described by the kernel $P_{Y|SXT}$ defined on $\mathbb{R}^{|\mathcal{Y}|\times|\mathcal{S}|\times|\mathcal{X}|\times|\mathcal{T}|}$. %furthermore, the relation between $U$ and the pair $(Y,X)$ is described by the kernel $P_{U|Y,X}$ defined on $\mathbb{R}^{|\mathcal{U}|\times|\mathcal{Y}|\times|\mathcal{X}|}$. 
In \eqref{eq:problem_1}, we consider the case where $r<H(X)$, otherwise it leads to the privacy-utility trade-off problems studied in \cite{kostala} and \cite{king3}. 
\begin{remark}
	\normalfont
	The trade-off in \eqref{eq:problem_1} can correspond to the privacy-utility trade-off with a rate constraint, as studied in \cite{gun}, incorporating an additional constraint where the Markov chain $(S,T)-X-Y$ holds. It is shown that when the rate constraint is inactive, i.e., $r$ is sufficiently large ($r\geq H(X)$) that the rate constraint is ignored, the problem leads to a linear program. In contrast to \cite{gun} we in this paper obtain new mechanism designs with active rate constraints. A simple scenario where the Markov chain $(S,T)-X-Y$ can be removed is to let $S$ and $T$ be deterministic functions of $X$.   
\end{remark}
The second problem which is closely related to the conditional fairness bottleneck problem in \cite{vari} can be stated as follows
%Therefore,
\begin{align}
g^{r}_c(P_{SXT})&=\sup_{\begin{array}{c} 
	\substack{P_{Y|SXT}:I(Y;S)=0,\\ \ \ \ \ \ \ \ \ \ I(X;Y|S,T)\leq r }
	\end{array}}I(Y;T|S),
    \label{eq:problem_2}
\end{align} 
The goal in the second problem is to design $Y$ that maximizes the information about the task which is not shared by the private data while satisfying the perfect privacy constraint and the bounded irrelevant data condition. In this work, the term \textit{irrelevant} corresponds to the part of the useful data $X$ which does not reveal information about the task $T$ and the private data $S$. 
\begin{remark}
	\normalfont
In \eqref{eq:problem_2}, in contrast to \cite{vari}, we relax the Markov chains $T-X-Y$ and $S-X-Y$ and assume that $X$, $S$ and $T$ are arbitrarily correlated. A simple scenario to remove the Markov chains is to let both $S$ and $T$ be deterministic functions of $X$, i.e., $S=f(X)$ and $T=g(X)$.	
\end{remark}



%For both design problems we use mutual information as utility and leakage measures. The privacy mechanism design problems for the two scenarios can be stated as follows %we define two privacy preserving functions $g_{\epsilon}(P_{XY})$ and $h_{\epsilon}(P_{XY})$ as follows 

 % which is assumed to be of full row rank. Thus, without loss of generality we represent $P_{X|Y}$ by two submatrices where the first submatrix is invertible, i.e., $P_{X|Y}=[P_{X|Y_1} , P_{X|Y_2}]$ such that $P_{X|Y_1}$ defined on $\mathbb{R}^{|\mathcal{X}|\times|\mathcal{X}|}$ is invertible. %$P_{X|Y}$ shows how much information about $X$ has been leaked to $Y$.
%Let $P_{X|Y}$ denotes the conditional distribution of random variables $(X,Y)$, which is represented by a matrix on
%Let $P_{X|Y}$ be represented by a matrix on  
%$\mathbb{R}^{\cal{K}\times\cal{K}}$, called kernel. Furthermore, we assume that the kernel is invertible. The key point to have a solution in privacy problem with perfect privacy described in \cite{
%1}, is that null space of the kernel should be non-empty, however here the null space of the kernel is empty, furthermore the kernel is invertible. The kernel denotes the privacy dependency between $X$ and $Y$.
 %The present work provides a framework where we unify these two results for a full row rank leakage matrix.
%This result was also proved in \cite{berger} in a source coding setup.
%The conditional distribution of $(X|Y)$ is represented by $P_{X|Y}$, where $P_{X|Y}$ is a matrix with size $|\cal{X}|\times|\cal{Y}|$, called channel matrix. Furthermore We assume that the channel matrix is invertible.
% The function $h_{\epsilon}(P_{XY})$ is used when the privacy mechanism has access to both the private data and the useful data. The function $g_{\epsilon}(P_{XY})$ is used when the privacy mechanism has only access to the useful data. Clearly, the relation between $h_{\epsilon}(P_{XY})$ and $g_{\epsilon}(P_{XY})$ can be stated as follows
%\begin{align}
%g_{\epsilon}(P_{XY})\leq h_{\epsilon}(P_{XY}).
%\end{align}
%In the following we study the case where $0\leq\epsilon< I(X;Y)$, otherwise the optimal solution of $h_{\epsilon}(P_{XY})$ or $g_{\epsilon}(P_{XY})$ is $H(Y)$ achieved by $U=Y$. 
% \begin{remark}
% 	\normalfont
% 	For $\epsilon=0$, \eqref{eq:problem_2} leads to the perfect privacy problem studied in \cite{borz}. It has been shown that for a non-invertible leakage matrix $P_{X|Y}$, $g_0(P_{XY})$ can be obtained by a linear program.
% \end{remark}
% \begin{remark}
% 	\normalfont
% 	For $\epsilon=0$, \eqref{eq:problem_1} leads to the secret-dependent perfect privacy function $h_0(P_{XY})$, studied in \cite{kostala}, where upper and lower bounds on $h_0(P_{XY})$ have been derived. 
% \end{remark}
 
